Model-free online motion adaptation for energy efficient flights of multicopters

Limited flight distance and time is a common problem for multicopters. We propose a method for finding the optimal speed and sideslip angle of a multicopter flying a given path to achieve either the longest flight distance or time. Since flight speed and sideslip are often free variables in multicopter path planning, they can be changed without changing the mission. The proposed method is based on a novel multivariable extremum seeking controller with adaptive step size, which is inspired by recent work from the machine learning community on stochastic optimization. Our method (a) does not require a power consumption model of the vehicle, (b) is computationally efficient and runs on low-cost embedded computers in real-time, and (c) converges faster than the standard extremum seeking controller with constant step size. We prove the stability of this approach and validate it through outdoor experiments. The method is shown to converge with different payloads and in the presence of wind. Compared to flying at the maximum achievable speed in the experiments with a uniformly selected random sideslip angle, flying at the optimal range speed and sideslip on average increases the flight range by 14.3% without payload and 19.4% with a box payload. In addition, compared to hovering, flying at the optimal endurance speed and sideslip increases the flight time by 7.5% without payload and 14.4% with a box payload. A video can be found at https://youtu.be/aLds8LVfogk.

==> sections/Sec2-Modeling.tex <==
\label{sec:modeling}
In this section we define the reference frames and briefly introduce the quadcopter dynamics, and the effects of flight speed and sideslip on the power consumption of the vehicle.
A power consumption model is given to help understanding some counter-intuitive effects observed in the experiments, e.g. the power consumption first decreases and then increases as the flight speed increases. 
This power consumption model is not used for the flight range and endurance optimization.

\subsection{Quadcopter dynamics}
\label{subsec:dynamics}
As shown in  \figref{figVehicleDiagram}, two sets of reference frames are defined --  an inertial frame $I$ attached to the ground and a body-fixed frame $B$.
The quadcopter is modeled as a rigid body with six degrees of freedom: three degrees of freedom from the linear translation and three degrees of freedom from rotation.
Each propeller $j$ ($j = 1, ..., 4$), produces a thrust $\mvec{f}_j$ and a torque $\mvec{\tau}_j$, both expressed in frame $B$.
\begin{figure}[h]
	\begin{center}
		\includegraphics[width =  \linewidth]{figures/Quad3D.pdf}
	\end{center}
% 	\vspace{-1ex}
	\caption{
		$I$ represents the inertial frame and $B$ represents the quadcopter's body frame. 
		We additionally show the thrust and torque from the $j$-th propeller $\mvec{f}_j$ and $\mvec{\tau}_j$, the free-stream velocity $\bm{v}_\infty$, the induced velocity $\bm{v}_i$, angle of attack $\alpha$, and the sideslip $\beta$, shown positive in the diagram.
	}
	\label{figVehicleDiagram}
\end{figure}
% latex symbols for this figure generated from https://viereck.ch/latex-to-svg/.

The orientation of the vehicle with respect to the free-stream velocity $\bm{v}_\infty$ is described by the angle of attack $\alpha$ and the sideslip $\beta$, as shown in \figref{figVehicleDiagram}. The angle of attack $\alpha$ is defined as the angle between ${\bm{v}_\infty}$ and the rotor plane; the sideslip is defined as the angle between $\bm{e}^B_1$ and the projection of ${\bm{v}_\infty}$ in the rotor plane. 

With $\mvec{x} \in \mathbb{R}^3$ and its derivatives denoting the translational position, velocity and acceleration of the vehicle, $\mvec{g}$ denoting the acceleration due to gravity, all expressed in the inertial frame $I$, the translational dynamics of the vehicle are given by
\begin{align}
m \mvecdd{x} &= m \mvec{g} + \mvec{R} \sum_j{\mvec{f}_j} + \mvec{f}_d, \label{eq:DynamicsTranslation}
\end{align}
where $\mvec{f}_d$ is the drag force and $\mvec{R}$ is the rotation matrix from the body frame $B$ to the inertial frame $I$. 
The drag force $\mvec{f}_d$ is a function of the rotation $\mvec{R}$ and free-stream speed $v_\infty$.
In addition, with $\mvec{\omega}$ and its derivative denoting the angular velocity and acceleration, expressed in the body-fixed frame $B$, the rotational dynamics of the vehicle is given by
\begin{align}
\mvecd{R} =& \mvec{R}\crossMat{\mvec{\omega}}, \\
\mvec{I} \mvecd{\omega} =& -\mvec{\omega}\times\mvec{I}\mvec{\omega} + \sum_j \mvec{\tau}_j, %+ \mvec{\tau}_d \label{eqDynamicsRotation}
\end{align}
where $\skewSym{\mvec{\omega}}$ is the skew-symmetric matrix form of the vector cross product.
%such that 
% \begin{align}
% \skewSym{\mvec{\omega}} = \mmat{0 & -\omega_3 & \omega_2 \\ \omega_3 & 0 & -\omega_1\\-\omega_2 & \omega_1 &0}.
% \end{align}
Control of the quadcopter is achieved by controlling the thrust and torque generated by each rotor. 
% \par
% Because the quadcopter is differentially flat
% \cite{differential_flatness}, any smooth trajectory with reasonably bounded derivatives in the space of the flat outputs can be followed by the multicopter.
% The translational position $\mvec{x}$ and yaw can be chosen as a set of flat outputs.
% So for applications where the multicopter is only required to follow a user-defined geometric path (i.e. position $\mvec{x}$ is specified), the yaw angle as well as the speed along the path will be free variables in generating a trajectory from the geometric path. \xiangyu{Not quite sure if we should add this paragraph. @Mark what do you think?}
% \par
A more detailed description of the quadcopter's dynamics and control can be found in e.g. \cite{tutorial}.


\subsection{Power consumption}
\label{subsec:power_cusumption}
When the flight speed increases, the power consumption of the vehicle usually first decreases and then increases.
This effect can be explained by the momentum theory \cite[Chapter 2.14]{leishman2006principles}.
% So to achieve the longest flight time, flying at a suitable speed is better than hovering.
% Following \cite{aerodynamics_control_multicopter} and \cite{ware2016analysis}, we assume that the vehicle's electrical power consumption $p_e$ (measured at the terminals of the battery) is proportional to the aerodynamic induced power $p_\text{induced}$,
% \begin{align}
% p_e = & \frac{1}{\eta}p_\text{induced},
% \label{eq:lumpedPowerConsumption}
% \end{align}
% where $\eta$ lumps the power losses from the battery to the propellers.
In forward flight, the propeller's power consumption $p$ is computed as 
\begin{align}
p = \kappa\mrb{v_i + v_\infty \sin\alpha} \sum_j \mnorm{\mvec{f}_j}_2, 
\label{eq:inducedPowerConsumption}
\end{align}
where $v_\infty$ = ${\mnorm{\mvec{v}_\infty}_2}$ is the magnitude of the free-stream velocity and $v_i$ represents the induced velocity applied by the propeller to the surrounding air.
%For simplicity we have assumed the angle of attack $\alpha$, the induced velocity $v$ and the freestream flow $\mvec{v}_\infty$ to be the same for every propeller, neglecting effects such as changes in freestream velocity due to non-zero angular rates $\mvec{\omega}$. 
The scalar $\kappa$ is an empirical correction factor.
The induced velocity $v_i$ is implicitly defined by
\begin{align}
v_i = \frac{v_h^2}{\sqrt{(v_\infty \cos \alpha )^2 + (v_\infty \sin \alpha + v_i)^2}},  \quad
v_h = \sqrt{\frac{mg}{8 \rho \pi r^2}},
\label{eq:InducedVelocity}
\end{align}
where $\rho$ is the density of the air and $r$ is the radius of the propellers. 
%A more detailed derivation and explanation of the power consumption model can be found in our previous work \cite{previous_paper_1}.

% Compared to hovering, flying at a low speed increases the free-stream velocity $v_\infty$ and decreases the induced power consumption. 
% When the speed is further increased, the drag force $\mvec{f}_d$ becomes significant and large motor thrusts are needed for the flight, which causes the increase in parasite power $p_p$ to outweigh the decrease in induced power $p_i$, causing the consumption to increase. 

Compared to hovering, flying at a low speed can help increasing the free-stream speed $v_\infty$ and decreasing the power consumption.
When the speed is further increased, the drag force $\mvec{f}_d$ becomes significant and large motor thrusts are needed for the flight, which cause power consumption to increase.
This effect can be validated by solving the equations \eqref{eq:inducedPowerConsumption} and \eqref{eq:InducedVelocity} numerically \cite[chapter 2.14]{leishman2006principles}.

In addition, because the vehicle is usually not perfectly axisymmetric (especially when carrying payload), flying at the same speed but with different sideslip produces different drag force $\mvec{f}_d$. This will cause the thrust forces $\mvec{f}_j$ to be different, leading to different power consumption. 
%So finding an efficient flight sideslip is also important for improving the flight range or endurance in addition to finding an efficient flight speed.
%This effect in forward flight was also observed by \cite{karydis2017energetics} and \cite{ware2016analysis}. 
